Fireiron: A Scheduling Language for High-Performance Linear Algebra on GPUs

Achieving high-performance GPU kernels requires optimizing algorithm implementations to the targeted GPU architecture. It is of utmost importance to fully use the compute and memory hierarchy, as well as available specialised hardware. Currently, vendor libraries like cuBLAS and cuDNN provide the best performing implementations of GPU algorithms. However the task of the library programmer is incredibly challenging: for each provided algorithm, high-performance implementations have to be developed for all commonly used architectures, input sizes, and different storage formats. These implementations are generally provided as optimized assembly code because performance-critical architectural features are only exposed at this level. This prevents reuse between different implementations of even the same algorithm, as simple differences can have major effects on low-level implementation details. In this paper we introduce Fireiron, a DSL and compiler which allows the specification of high-performance GPU implementations as compositions of simple and reusable building blocks. We show how to use Fireiron to optimize matrix multiplication implementations, achieving performance matching hand-coded CUDA kernels, even when using specialised hardware such as NIVIDA Tensor Cores, and outperforming state-of-the-art implementations provided by cuBLAS by more than 2x.

==> tex/design.tex <==
\begin{enumerate}
        \item Allow authoring and arbitrary composition of “distributed operations,” such as an algorithm CTA-wide reduction.
                These reusable operations need to assume that, say, their inputs are values distributed in registers of a CTA.
                Code modules that expect values in registers are not easily reusable in CUDA.
                =⇒ Distributed data structures serve as inputs to these operations.
                The code generator composes the operations and maps the distributed operations to physical storage elements.
        \item Get fusion for free.
                Sidestep the need for a dedicated fusion compiler transformation.
                =⇒ If operations communicate via a distributed data structure that resides in registers, these two operations are fused (because two operations cannot be “closer together” than passing a value via registers).
                This view allows us to generalized fusion to weak fusion, where operations might communicate via shared memory.
        \item Programmer can control aspects of the implementation strategy when desired.
                She can override the synthesizer or impose an optimization not known to the synthesizer.
                =⇒ Sketches allow leaving layout unknown, or you can replace a default (tiled) implementation of a subspec with a very different strategy.
        \item Important implementation concerns must (1) be first-class concepts in the language and (2) be specifiable in the strategy before less important decisions are made.
                This must be true whether the program is written manually, by a synthesizer, or a mix of both.
                =⇒ Floor-planning decisions such as how DN weights are stored across the GPU 1 must be trivial to state, and the remainder of the implementation should just follow this constraint.
                Alternatively, it must be possible to state a communication strategy, with rest following from this constraint.
        \item Compile to existing optimized code fragments, not just to low-level instructions.
                Fragments can range from HMMA to an optimized DN cell.
                This requirement is dual to floor-planning, where we do give the top-level decomposition, rather than target a leaf-level specification.
                =⇒ Ask the synthesizer to produce layouts and tile shapes to reduce a spec to a target fragment, which will have its own spec.
        \item Expose GPU compute and storage resources but delegate index computation to code generator.
                Programs have control over mapping of data to the memory hierarchy (registers, shared memory, and so on), as well as mapping of computations to the compute hierarchy (threads, warps, CTAs).
                But the CUDA indexing variables such as blockIdx are hidden from the programmer.
                =⇒ The code generator translates the mapping from data/code to the hardware into CUDA index computations.
        \item No restrictions on perfect loop nests.
                The programmer can include arbitrary operations as long as we can check their correctness wrt their spec with a solver.
                =⇒ We can already insert loads and stores into arbitrary places.
                There may be a need for if statements, too.
        \item Decompose the synthesis problem into smaller subproblems.
                =⇒ Compose larger implementations from smaller ones.
                Enabled by the hierarchical representation.
        \item Burn storage, not cycles.
                Rather than recompiling a program, find efficient strategies for its subcomponents and store them in persistent storage for lookup during future compilations.
                =⇒ Decomposing a program into hierarchical subproblems allows this reuse.
        \item Discover what subproblems would be useful for a given problem.
                This is dual to targeting a particular efficient operation.
                =⇒ This might be able to discover new distributed operations useful for a particular workload.
\end{enumerate}



==> tex/flaws.tex <==
The current implementation of Fireiron contains several flaws an limitations explained in the following:

\paragraph{Fixed Arity for Specs}
Every Spec is defined/seen as an operation $c = f(a,b)$, e.g., $c = \text{matmul}(a,b)$.
This means, that every Spec contains three Matrices (A,B and C) which does not make sense for Moves where you only have two matrices (src, dst)

\paragraph{Fixed Operations for Specs}
The operations each Spec needs to implement are specified in the abstract class Spec. The way it is currently implemented is that the union of all required operations is gathered in the spec class.
Therefore, Move also needs to implement Split for example which absolutely does not make sense and is avoided with specifying ???

\paragraph{Tiling Operations specific for each Spec}
We should probably add a generic partition functionality for Tensors and the define tile and split using this partition function

\paragraph{Names} \emph{Tile} and \emph{Split} are highly confusing. The difference for Matmul is not necessarily clear

\paragraph{Data Layout Specific for Matrices:} Layout is fixed to RowMajor/ColMajor but when we're talking about tensors it should be HWTN (or whatever letters they used)

\paragraph{Continuation-passing Style IR Construction}
The IR tree is constructed in continuation-passing style which is most likely more complicated than it could be.
The problem is, that every node contains a child, the node which implements the subproblem, which is not known at the time of creation of the parent.

Maybe we can work around this with using this off-by-one construction which contains a root node?

\paragraph{Accumulating MM via split}
Currently, a valid MM decomposition needs to contain split since the leaf node is written as an accumulating matrix multiplication which only exists after the first application of split.

\paragraph{Epilog}
Epilog specification is somewhat counter intuitive because it needs to be specified on the block level before we decomposed the computation to threads.
At least for matrix multiplication we kind of need two block-level decompositions, the compute-decomposition and epilog -decomposition (maybe three if you count init).
Compute-decomposition describes which thread computes which elements of C and where they are stored in registers.
If Compute and Epilog decomposition mismatch, which they will often do, we somehow need to arrange results in shared memory first before we can write them back to global memory.
Not trivial to infer this, somehow need to find a nice api to specify predication of threads.

\paragraph{Array Index Computation}
Array indices are computed by concatenating strings which makes it infeasible to do arithmetic simplification (0 * N = 0) or remove unused, wrong parameters, when doing predication.
Need to replace this with some symbolic AST (not too powerful but which allows to do some simple manipulations)

\paragraph{Mutability}
Code generation uses a lot of mutable variba

\paragraph{Redundancy}
The same API, tile split etc, needs to be implemented by FluentIR AND specs.
FluentIR creates the IR nodes and specs create subspecs of themselves.

\paragraph{Static Array Sizes}
For now we require to know all array sizes statically and we require that tile sizes evenly divide array sizes.

\paragraph{Codegen}
Index computations are computed using a data structure Env which always indices for three arrays even though that seldom makes sense, lots of ??? in the code.


==> tex/goals_ras.tex <==
We have four goals that are each supported with a new mechanism.

%-----------------------------------------------------------------------------------------------------------------------
% G O A L  1
%-----------------------------------------------------------------------------------------------------------------------
\subsection{Goal 1: Optional manual control over the implementation strategy.}
We offer the kernel programmer the ability to override the strategy produced by the compiler and impose his own strategy.

\paragraph{Mechanism:}
The programmer specifies the strategy using a strategy language.
This language controls the decomposition of the MM problem, the placement of data onto the memory, the communication of data, as well as the mapping of computations onto the compute elements.
In more detail, the implementation is generated by applying the strategy on the specification of the original kernel (which is a MM of a particular size).
The result is the implementation.
\begin{center}
strategy(spec) −→ impl
\end{center}

%-----------------------------------------------------------------------------------------------------------------------
% G O A L  2
%-----------------------------------------------------------------------------------------------------------------------
\subsection{Goal 2: Reuse of implementation strategies.}
We offer the kernel programmer to reuse previously developed strategies, including those that cannot be reused by calling a library procedure.

\paragraph{Mechanism:}
The implementation is hierarchical and each fragment of the implementation can be described with a concise specification.
These specifications can be implemented with strategies that can be stored as first-class objects and reused.
In more detail, the implementation is a strategy tree whose leaves are specifications of subcomputations.
In a final implementation, the leaves are instructions or library kernels. In a partial implementation, the leaves can be specifications that need to be implemented (or decomposed into a strategy).
Imagine we want to implement a kernel with the specification spec.
If we apply a partial strategy, we might obtain n implementation whose leaves are specifications spec 1 and spec 1 :
\begin{center}
strategy 0 (spec 0 ) −→ impl 0 (spec 1 , spec 2 )
\end{center}
We next implement these two leaf specifications, applying on them strategies strategy 1 and strategy 2, respectively:
\begin{center}
impl 0 (strategy 1 (spec 1 ), strategy 2 (spec 2 )) −→ impl 0 (impl 1 , impl 2 )
\end{center}
This results in replacing spec 1 with impl 1 in the implementation spec 0 , and the same for spec 2 .

%-----------------------------------------------------------------------------------------------------------------------
% G O A L  3
%-----------------------------------------------------------------------------------------------------------------------
\subsection{Goal 3: Target instructions with arbitrary granularity.}
The strategy language must create implementations that use machine instructions, macro instructions such as WMMA, and kernel libraries such as cuBLASS.
The instructions can manipulate low-level hardware state, such as the content of the register collector and other software controlled caches.
\paragraph{Mechanism:}
Instructions, macro-instructions, and kernels are specified with the same kind of specifications as the top-level specifications and the intermediate specifications.
In more detail, if the implementation impl 0 (spec 1 ) is such that its leaf specification spec 1 equals the specification of the instruction FMA, then the implementation is complete because all of its leaf specifications are executable.
\begin{center}
impl 0 (spec 1 ) ∧ spec 1 = spec(FMA) ⇒ impl 0 (spec 1 ) is executable.
\end{center}

%-----------------------------------------------------------------------------------------------------------------------
% G O A L  3
%-----------------------------------------------------------------------------------------------------------------------
\subsection{Goal 4: Data types for parallel cooperation. }
In parallel programs, multiple threads cooperate to (1) load an array, (2) compute its values, and (3) store it back. In advanced implementations, the mapping of the array elements to threads may change between the three phases.
To simplify programming such implementations, we want to abstract away from the mapping as long as possible, specifying it only at the lower level of the strategy.
This makes higher-level specifications more abstract, permitting more possible implementations.
\paragraph{Mechanism:}
Distributed arrays are data types that the programmer can distribute onto private memories.
Fireiron provides the illusion that a distributed array is indivisibly stored across, say, registers of multiple warps; here, registers are memories that are private to each thread.
The Fireiron compiler divides the array and distributes the pieces onto registers of threads of the involved warps.
In more detail, the mapping of a distributed array onto private memories is viewed as a generalized memory layout.
In normal layout, a 2D matrix can be mapped to 1D memory in row-major order, or in column-major order. This mapping is a function from element index space to meory address space.
In the generalized layout, a matrix is divided according to a tiling pattern, and the tiles are mapped onto private memories of thread blocks or threads.
The mapping is a function from tile coordinate space to thread (or thread block) coordinate space.
At the next level of the hierarchy, the tile elements are mapped to 1D memories as in the normal layout.


==> tex/impl.tex <==
Here I describe how the new features are described technically.

\paragraph{IR construction}
Keeping FluentIR continuation passing style for now. As an alternative it should also be possible to construct the IR fully manually by constructing the tree completely from scratch: Tile(spec, size, Tile(??, size2, Load(...).
Maybe not.

Introducing Decompositions (old FluentIR) and Refinements (started with FluentTile).
Basically a Decomposition creates a new node in the IR whereas a Refinements provide a concise API to change certain parts of the current IR node.
Also, Refinements are Node specific which is nice, hopefully

Specs -> LayerSpec, accept LayerSpec as input instead of Matrix. Matrix is itself a LayerSpec (e.g., InputLayer). What does that mean for decomposition? CodeGen? .load?
That makes it difficult to "load" them to different locations in the memory hierarchy if the thing to load is not a matrix

Trying to write minimal working example of GEMM

\subsection{Decomposition}
A \emph{Decomposition} is a simple function $d:\text{Spec} \rightarrow \text{Spec}$.
Every decomposition has one of three purposes:
\begin{itemize}
        \item{Descend in the memory hierarchy}
        \item{Descend in the compute hierarchy}
        \item{Combine decompositions}
\end{itemize}

It is yet unclear how to ascend the hierarchies again.
In v1 it was a big hack using .epilog.
What is a better way of specifying our way up again?
The following is a brief explanation of all operations currently supported to decompose Specs.

\paragraph{Tile}
\texttt{Tile(size: (Int, Int))} expects a shape (currently \texttt{Int}-tuple, \texttt{Shape} in Fireiron v1) and returns a "smaller" spec of the same computation type (MM, Move, ...).
Matrices of the argument spec are tiled according to the semantics of the given operation.
For MM, C will be updated to have given size, A's rows and B's cols are tiled accordingly.
For Move, both \texttt{src} and \texttt{dst} are set to the given size.

Tile offers optional \emph{Refinements}:
\begin{itemize}
        \item \texttt{.to(level: ComputeHierarchy)} changes the assignment of the current compute hierarchy. If unspecified, the new spec has the same assignment as the old spec.
        \item \texttt{.threadLayout(layout: ThreadLayout)} specifies how the created tiles are assigned to the thread's IDs (\texttt{*Idx.x} and \texttt{*Idx.y}).
                \begin{itemize}
                        \item \texttt{ThreadLayout.RowMajor}: \texttt{*Idx.x} iterates over the created row tiles
                        \item \texttt{ThreadLayout.ColMajor}: \texttt{*Idx.x} iterates over the created column tiles
                \end{itemize}
        \item \texttt{.swizzle(swizzle: String => String} changes how the \texttt{linearID} (computed using \texttt{*Idx.x} and \texttt{*Idx.y}) accesses linear memory.
\end{itemize}

\paragraph{Split}
\texttt{Split(size: Int)} is MM-specific and specifies that the k-dimension shall be tiled (sometimes called \emph{split-k}, hence the name).

\paragraph{Load}
\texttt{Load(array: Int, location: MemoryHierarchy, impl: Decomposition)}
expects an array, a location in the memory hierarchy and a decomposition which explains how to load \texttt{array} into the given \texttt{location}.

\paragraph{Then}
\texttt{Then(fst: Decomposition, snd: Decomposition)} (operator: \texttt{|>}) combines two strategies sequentially. For example \texttt{Tile((64,64)) |> Tile((32,32))}

\paragraph{Epilog}
\texttt{Then(initLoc: MemoryHierarchy, initDec: Decomposition, epilogDec: Decomposition}
Problem with the epilog: How is it defined as a function from spec to spec?

\paragraph{Done}
\texttt{Done()}
asdf

\paragraph{Debug}
\texttt{Done()}
asdf



\paragraph{Conclusion}
These building blocks can be combined to arbitrary decompositions.
Once a decomposition is applied on a spec, types are checked.
This allows to restrict the usage of


==> tex/intro_ras.tex <==
When implementing high-performance applications, GPU programmers rely extensively on libraries of fine-tuned subroutines such as cuBLAS and cuDNN.
One limitation of today’s libraries is that their subroutines must be invoked as procedures.
In particular, inputs to these implementations must be passed as procedure arguments.
While it is possible to pass to procedures addressable objects that are stored in global memory or in shared memory, it is not possible to pass an array that is stored, for example, in registers or in FMA argument collectors, whose address cannot be taken.
This restriction prevents the library from decomposing existing implementations into flexible smaller components from which a new efficient implementations could be composed by the user of the library.

For example, the user may want to implement a matrix multiplication that finds its input matrices stored in registers.
The benefit of such an implementation is that it can be fused with the operations that produced the matrices.
The fusion happens because the implementation need not load the matrices from the memory to registers; the matrices are already in registers when the implementation is called.
Inputs stored in registers pose a problem for today’s libraries because registers names cannot be passed to parameterize an implementation at runtime; the names need to be code-generated at compile time.

Consider the case when the input matrices are distributed across the registers of the threads of a cooperative thread array (CTA).
Ideally, we want to specify the location of the matrix (in registers) when calling the library procedure.
However, today, the procedure needs to be compiled for a particular size of the matrix and a particular number of threads in the CTA.
Additionally, the implementation of the producers of the matrices needs to be coordinated so that the matrices are placed in the registers expected by the consumers.
This coordination prevents independent development and reuse of implementations, making libraries less useful than they could be.
We describe a compiler architecture that allows breaking existing efficient library procedures into reusable pieces.
Example of such reusable components include:
\begin{itemize}
        \item  parallel matrix multiplications whose data resides in registers,
        \item  parallel data move operations where multiple threads cooperate to load data from global memory to shared memory via registers.
\end{itemize}
Our compiler architecture allows reusing such implementations as so-called implementation \textit{decompositions}, rather than as code.
A \textit{decomposition} describes how a computation (for example a matrix multiplication or a data transfer) should be implemented.
Part of the decomposition is a description of where the inputs are located, i.e., how they are distributed across registers or other physical storage locations of multiple threads.
The user writes the decomposition using a small number of \textit{scheduling instructions} that comprise the scheduling language.
The compiler uses the decomposition to transform the source code (given as a specification of what logical computation we wish to achieve) into an implementation described in the strategy.
Importantly, unlike procedures of today’s libraries, the decompositions are composable: the user can put together a strategy that loads matrices into registers with a strategy that multiplies these register-resident matrices.
At the technical level, the strategy instructions accept the original specification and decompose it into smaller specifications.
On these smaller sub-specification, the compiler can apply other strategies.
A reuse is possible whenever the compiler creates a sub-specification that matches an existing decomposition.

\subsection{Some Terminology}
\begin{itemize}
        \item Specification: A spec describes what a program computes. The signature includes everything we need to know to implement a specification, from the shapes of the parameters to their layout in memory.
        \item Implementation: A program that implements a specification.
        \item Strategy: An implementation strategy translates a spec into its implementation.
        \item Fluent transforms: Functions that apply a strategy, transforming a spec into a partial implementation.
        \item Sketch: A program with unknown parts that are to be synthesized.
\end{itemize}

\subsection{Notable Properties}
\begin{itemize}
        \item Distributed data structures: Matrices distributed across storage elements not accessible to all threads of a program.
                For example, a matrix can be stored in registers of all threads of a CTA.
        \item Hierarchical programs: Programs are composed of nested specifications.
                For example, a matrix multiply kernel may invoke a matrix multiple of smaller matrices.
        \item Synthesis: Implementations can be produced automatically to meet a desired specification.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
Fireirons main motivation:
\begin{itemize}
        \item Easily change the implementation/optimization for high-performance ML operations by defining reusable optimizations as combinations of \emph{Decompositions}.
                Enabling performance experts to quickly experiment with different implementations.
        \item First, full control to the developer, second somehow automate parts of it? Explore some spaces?
        \item Allow to store/reuse known high-performance implementations for specs, e.g., a warp-level matmul on kepler.
                Should be easy to plug in these implementations for specific Specs to make use of performance expert knowledge.
        \item Store some decompositions as reusable optimization implementations (e.g., crosswise-prefetching from GL to SH)
\end{itemize}




==> tex/ir.tex <==
Fireiron has two intertwined IRs: specifications and implementations.
Specifications describe what is to be computed, while the implementations describes how a computation proceeds.
In other words, the specification is the problem and an implementation is a solution to the problem (an algorithm that solves the problem).
In Fireiron, it is possible to check whether an implementation correctly implements a specification.

%-----------------------------------------------------------------------------------------------------------------------
% S P E C I F I C A T I O N S
%-----------------------------------------------------------------------------------------------------------------------
\subsection{Specifications}
A specification has a logical (mathematical) part, and a physical (implementation) part.

\begin{itemize}
        \item The logical part describes the mathematical operation that is to be performed on the input matrices.
        \item The physical part describes how the logical matrices are mapped to the physical memory hierarchy.
                This part of the specification includes everything that an implementation may need to know about the input and output matrices.
\end{itemize}

%-----------------------------------------------------------------------------------------------------------------------
% M A T M U L
%-----------------------------------------------------------------------------------------------------------------------
\paragraph{Example: A specification of a matmul problem}
The following code is a specification of a matrix multiplication problem C := A ∗ B.
The specification gives the properties of the matrices: their dimensions; the type of their elements; and the level of the memory hierarchy in which the matrices are stored, here, it is the global memory (GL).
It is assumed that the matrices A, B, and C are allocated by the caller.
The last argument specifies that the implementation should be executed on all threads of a thread block (as opposed to all thread blocks, or a warp, or a single thread).

MM ( A : Matrix (128 , 8 , GL , Float ) ,
B : Matrix ( 8 ,128 , GL , Float ) ,
C : Matrix (128 ,128 , GL , Float ) ,
ThreadBlock )

The following elaborates on the parameters of a specification.

%-----------------------------------------------------------------------------------------------------------------------
% F U N C T I O N S
%-----------------------------------------------------------------------------------------------------------------------
\paragraph{Functions}
Fireiron specifications compute just one of two functions: a matrix multiply and a move operation. These two operations are sufficient to implement advanced matrix multiply implementations.
\begin{itemize}
        \item MM(A,B,C): A matrix multiplication C := A ∗ B. There is a variant of MM called MM+ which performs C += A ∗ B, that is, it increments the value of C by A ∗ B.
        \item  MOVE(A,C): This specification asks the implementation to perform a physical copy of matrix C to the matrix A.
                Instructions that implement MOVEs include stores, loads, and register-to-register copies.
                MOVEs are typically used to move tiles of matrices between the levels of memory.
\end{itemize}

Note that moves may have advanced implementations.
For example, a matrix stored in registers of a warp may be moved to global memory via shared memory.
Such specification is decomposed into two moves: one from registers to shared memory, followed by another from shared memory to global memory.

%-----------------------------------------------------------------------------------------------------------------------
% P A R A M E T E R S
%-----------------------------------------------------------------------------------------------------------------------
\paragraph{Parameters}
A specification has one or two input parameters, and one output parameter.
All parameters are 2D matrices.
The input of MMs specifications are named A and B; the input of MOVEs are named A.
Specifications have one output parameter named C.

%-----------------------------------------------------------------------------------------------------------------------
% T Y P E S  O F  P A R A M E T E R S
%-----------------------------------------------------------------------------------------------------------------------
\paragraph{Types of Parameters}
Parameters of specifications are 2D matrices. The static type of a matrix includes the following information:
\begin{itemize}
        \item The type of matrix elements: int, float, double, etc.
        \item The shape of the logical matrix, given as the sizes of the two logical dimensions.
                Currently, the sizes are constants known at compile time.
        \item The physical memory in which the matrix is stored. Currently, it is one of GL (global memory), SH (shared memory), RC (register cache), or RF (register file).
        \item The layout of the logical matrix in physical memory. The layout is a function that maps logical indices to 1D physical memory. Currently, we support layouts RM (row major), CM (column major), in combination with padding, which will offset each row or column.
\end{itemize}


==> tex/language.tex <==
\begin{figure*}
        \includegraphics[width=\linewidth]{img/boxes}
        \caption{Pseudocode GPU implementation of a matrix multiplication.
        Conceptually a matrix multiplication operation is decomposed multiple times into smaller matrix multiplications.
        By descending the compute and memory hierarchy, eventually a single thread multiplies two elements residing in registers}
        \label{fig:boxes}
\end{figure*}
Most problems are \emph{decomposable} into smaller problems of the same kind.
Figure \ref{fig:boxes} visualizes this property using the example of a simple kernel implementing matrix multiplication.
At the beginning of the kernel, the input matrices A ($M\times K$), B ($K \times N$) and C ($M \times N$) reside in global memory (simply denoted as \texttt{MatMul(M,N,K)(GL,GL,GL) (Kernel))}.
By creating tiles of size $128\times128$, smaller instances of the same operation (matrix multiplication) are created are computed by a single thread-block denoted as \texttt{(MatMul(128,128,K)(GL,GL,GL)(Block))}.
This continues until we assigned a tile of certain size to each thread of each warp while specifying when to change the location of data within the memory hierarchy in the meantime.

Fireiron exploits this idea and makes use of two main concepts: \emph{Specifications} and \emph{Decompositions}

\subsection{Specifications and Decompositions}
A Specification (in the following briefly \emph{spec}) describes \emph{what} a program computes.
A Spec contains everything we need to know to implement the operation.
This especially entails that a Spec keeps track of the shapes, locations and storage layouts of its input and output matrices, as well as which level of the compute hierarchy (i.e., Kernel, Block, Warp or Thread) is responsible for computing this operation.

Currently we support two main specs:
Matrix Multiplication (MatMul) and data movement (Move) from one level of the memory hierarchy to another.

A \emph{Decomposition} describes \emph{how} to implement a given spec.
More specifically, a decomposition is a function $d: Spec \rightarrow Spec$ which given a spec returns a new spec.
Currently we provide a small set of composable decompositions:
\begin{itemize}
        \item \texttt{spec.tile(r, c)} creates $r\times c$ shaped tiles in output matrix, tiles in the input are created accordingly.
        \item \texttt{spec.split(s)} splits the k-dimension of A and B into chunks of size $s$. (Currently only defined for MatMul specs)
        \item \texttt{spec.load(m, l, d)} loads the matrix $m$ to location $l$. By creating a Move spec which is decomposed with the given decomposition $d$.
        \item \texttt{spec.done}
\end{itemize}
Currently, a spec contains Matrices (eventually Tensors) and an assignment to a level of the Compute Hierarchy specifying who is responsible for computing this problem (i.e., Kernel, Block, Warp, Thread)

\begin{lstlisting}
mm = MatMul(M,N,K)(GL,GL,GL)(Kernel)
mm.tile(128,128).to(Block) //MatMul(128,128,K)(GL,GL,GL)(Kernel)
  .epilog(RF, init, store) //MatMul(128,128,K)(GL,GL,RF)(Kernel)
  .split(8)                //MatMul(128,128,8)(GL,GL,RF)(Kernel)
  .load(A, SH)             //MatMul(128,128,8)(SH,GL,RF)(Kernel)
  .load(B, SH)             //MatMul(128,128,8)(SH,SH,RF)(Kernel)
  .tile(64,32).to(Warp)    //MatMul(64 , 32,8)(SH,SH,RF)( Warp )
  .tile(8,8).to(Thread)
  .split(1)
  .load(A, RF)
  .load(B, RF)
  .tile(1,1)
  .done
\end{lstlisting}

\subsection{Scheduling Language / FluentIR}
Fireiron's operations defined on Specs are inspired by Halides scheduling language.
Fireiron provides a small set of operations applicable to specs to refine the current problem.
Currently, the following operations exist: tile, split, load, leaf

\subsubsection{Tile}
Basic building block to decompose the current problem into smaller sub-problems.

\subsubsection{Split}
Specific for matrix multiplication: Splitting k-dimension to reduce pressure on shared memory

\subsubsection{Move}
Copy src matrix to dst matrix

\subsubsection{Extension}
Can we already foresee which extensions to the operations we need most likely? What about fusion? What about convolution? What about computation graphs as input?
Check implementations of high-performance ML operators.
Check HLA, TVM, Nvidia-internal Matmul (XMMA) and Conv implementations.

What about the trove and multpoly benchmarks? These could be used in a paper!

\subsubsection{Epilog/Init/Store}
Specify how to write back the results residing in registers to GL. Multiple problems here

A strategy transforms a specification into an implementation. A strategy is composed from steps, each of
which creates just one node of the implementation. The four key strategy steps are below:
\begin{itemize}
        \item s.tile(shape): Decomposes the specification s by partitioning the output. The shape parameter gives the size of the output tile.
                This transformation applies to both MM and MOVE.
                For MOVEs, the step creates a TileLoop that decomposes the MOVE across multiple threads/warps/blocks.
        \item s.split(shape): Decomposes the specification s by partitioning the input matrix(es).
                The shape parameter gives the size of the input tile in the parameter A.
                This transformation applies to both MM and MOVE.
                For MMs, this step creates a SplitLoop that implements the matrix multiplication using the outer product algorithm.
                See the discussion of the SplitLoop above.
        \item s.load(A/B,mem): Moves the argument A or B of the specification s into the memory mem, then invokes s.
                This transformation creates a new matrix in memory mem with the same shape as that of A/B.
                It also changes the signature of the specification s to account for its parameter now residing in memory mem
        \item s.store(mem): Analogous to .load except it creates a matrix for the output of s, which is MOVEd to C after s finishes.

\end{itemize}



==> tex/milestones.tex <==
\begin{enumerate}
        \item Finish IR and Codegen refactoring and support as many features as we did during the internship. Steps required in order:
                \begin{itemize}
                        \item \sout{Redesign decompositions as small composable language instead of "Fluent" interface}
                        \item \sout{Create similar AST to the one we had before using a "decomposition program"}
                        \item \sout{Implement index computation using simple ArithExpr IR instead of concatenating strings}
                        \item \sout{Generate simple but correct "Hello-World"-MM kernel}
                        \item \sout{Support row- and column-major storage for matrices}
                        \item \sout{Support vectorized loads (similar to supporting XMMA)}
                        \item \sout{Support strided shapes}
                        \item Support Epilogue (better way to do this than what we did before?)
                        \item \sout{Support swizzle expressions}
                        \item Re-implement swizzle visualization (reuse old?)
                        \item \textbf{Deadline: 09. January}
                \end{itemize}
        \item Reach at least 95\% performance of Andrew Kerrs Maxwell GEMM code
                \begin{itemize}
                        \item Figure out how to express complex epilogues with temporary buffer in shared memory.
                        \item Investigate performance regressions (Fireiron's kernels where slower for yet unknown reasons)
                        \item \textbf{Deadline 23. January}
                \end{itemize}
        \item Finish Intro/Motivation/IR/Codegen section of techreport. Some problems are still open here. E.g., how to specify the Epilog in Fireirons decomposition language? Compare to Cutlass. List to check items off:
                \begin{itemize}
                        \item Get access to Ras' document
                        \item Intro
                        \item Motivation
                        \item IR
                        \item Codegen
                        \item Preliminary results
                        \item \textbf{Deadline 30. January}
                \end{itemize}
        \item Familiarize with advanced optimization techniques: XMMA, Scott Grays GEMM code, Double-buffering, whatever Cutlass uses to make their kernels run fast
                \begin{itemize}
                        \item Investigate XMMA
                        \item Understand Andrews and Scott Grays double buffering implementation
                        \item Investigate Cutlass
                        \item Quite imprecise, Use these insights to create new milestones!
                        \item \textbf{Deadline 06. Februar}
                \end{itemize}
\end{enumerate}


==> tex/motivation.tex <==
In order to implement any operation in an efficient way on a GPU, we need to find optimal solutions to multiple problems at the same time:
How to assign data of our input matrices to the different elements of the compute hierarchy?
How many element shall be computed by a single thread?
How to move data between different layers of the memory hierarchy?
Which storage layouts are the most efficient for each of our inputs?

Experimenting with different implementations is difficult since...
Fireiron allows to gradually design an implementation of the operation while iteratively refining this implementation.

\subsection{Assigning Data to Threads}
As a first step, we need to decide how to map input data elements to the different levels of the compute hierarchy.
That means, we need to decide how many elements are computed by a single block, warp and thread.
Instead of computing an entire row of C at a time, tiling causes the computation to process by rectangular tiles in C.
To do this, Fireiron provides the \texttt{.tile} decomposition.
These tiles can be assigned to a specific level of the compute hierarchy using \texttt{.to}:

\begin{lstlisting}[style=fireiron]
// mm = MatMul(M,N,K)(Kernel)
mm.tile(128,128).to(Block) // MatMul(128,128,K)(Block)
  .tile(64,32).to(Warp)    // MatMul(64,32,K)(Warp)
  .tile(8,8).to(Thread)    // MatMul(8,8,K)(Thread)
  .tile(1,1)               // MatMul(1,1,K)(Thread)
\end{lstlisting}

\subsection{Outer Product Blocked Matrix Multiplication}
Each element in these tiles still requires a full row of A and a full column of B, both of size $K$.
Instead, we need another level of tiling and divide $K$-dimension into smaller chunks to eventually be able to load those into lower levels of our memory hierarchy.
To do this, Fireiron provides the \texttt{.split} decomposition:

\begin{lstlisting}[style=fireiron]
// mm = MatMul(M,N,K)(Kernel)
mm.tile(128,128).to(Block) // MatMul(128,128,K)(Block)
  .split(8)                // MatMul(128,128,8)(Block)
  .tile(64,32).to(Warp)    // MatMul(64,32,8)(Warp)
  .tile(8,8).to(Thread)    // MatMul(8,8,8)(Thread)
  .split(1)                // MatMul(8,8,1)(Thread)
  .tile(1,1)               // MatMul(1,1,1)(Thread)
\end{lstlisting}

\subsection{Prefetching Data to Exploit Memory Hierarchy}
Further, we'll extensively prefetch data from global memory into shared memory and from shared memory into registers.
To do this, Fireiron provides the \texttt{.load} decomposition:

%// MatMul(128,128,K)(GL,GL,GL)(Block)
%// MatMul(128,128,8)(GL,GL,GL)(Block)
%// MatMul(128,128,8)(SH,GL,GL)(Block)
%// MatMul(128,128,8)(SH,SH,GL)(Block)
%// MatMul(64,32,8)(SH,SH,GL)(Warp)
%// MatMul(8,8,8)(SH,SH,GL)(Thread)
%// MatMul(8,8,1)(SH,SH,GL)(Thread)
%// MatMul(8,8,1)(RF,SH,GL)(Block)
%// MatMul(8,8,1)(RF,RF,GL)(Block)
%// MatMul(1,1,1)(RF,RF,GL)(Thread)

\begin{lstlisting}[style=fireiron]
// mm = MatMul(M,N,K)(Kernel)
mm.tile(128,128).to(Block)
  .split(8)
  .load(MatMul.A, SH, _)
  .load(MatMul.B, SH, _)
  .tile(64,32).to(Warp)
  .tile(8,8).to(Thread)
  .split(1)
  .load(MatMul.A, RF, _)
  .load(MatMul.B, RF, _)
  .tile(1,1)
\end{lstlisting}





\paragraph{Tiling}


